Spectral symmetry fingerprints in equivariant representations

Symmetry governs the organization of physical structures, while symmetry breaking reveals their transformations. In geometric deep learning, symmetry imposes rank constraints on equivariant representations, limiting the expressive capacity of equivariant graph neural networks (GNNs). Here we show that these constraints can instead be exploited: the singular-value spectra of equivariant representations provide a unified fingerprint of structural symmetry. We introduce spectral symmetry fingerprints (SymFP), which enable discrete point-group identification through rank-template matching and continuous symmetry analysis by quantifying spectral energy beyond target rank constraints. SymFP is orientation invariant and architecture agnostic, enabling a parameter-free GNN implementation. Its spectra can be reused across multiple target groups, and the resulting leakage scores satisfy subgroup monotonicity. Across synthetic structures, molecules, coordination complexes and large biological assemblies, SymFP accurately identifies point groups, tracks controlled symmetry breaking and reveals local and degree-resolved symmetry changes that can be obscured by global geometric measures. These results establish the spectral structure of equivariant representations as a general framework for characterizing symmetry across physical systems.

==> latexmkrc <==
$pdf_mode = 1;

# bibunits writes one bu<N>.aux per reference list and latexmk knows nothing about
# them, so without this the two bibliographies come out empty on any stock latexmk
# setup, Overleaf included. Running bibtex over them after every pdflatex pass is
# enough, since latexmk keeps passing until the aux files stop changing.
$pdflatex = 'internal pdflatex_with_bibunits %O %S';

sub pdflatex_with_bibunits {
    my $ret = system('pdflatex', '-shell-escape', '-interaction=nonstopmode', @_);
    foreach my $aux (glob('bu*.aux')) {
        my $base = $aux;
        $base =~ s/\.aux$//;
        system('bibtex', $base);
    }
    return $ret;
}

